Noise-Sustained Convective Instability in a Magnetized Taylor-Couette Flow

The helical magnetorotational instability of the magnetized Taylor-Couette flow is studied numerically in a finite cylinder. A distant upstream insulating boundary is shown to stabilize the convective instability entirely while reducing the growth rate of the absolute instability. The reduction is less severe with larger height. After modeling the boundary conditions properly, the wave patterns observed in the experiment turn out to be a noise-sustained convective instability. After the source of the noise resulted from unstable Ekman and Stewartson layers is switched off, a slowly-decaying inertial oscillation is observed in the simulation. We reach the conclusion that the experiments completed to date have not yet reached the regime of absolute instability.

==> response.tex <==
% This response to the referee is written in plain TeX (not LaTeX)
%
\magnification=\magstep1
\centerline{\bf Revisions to ApJ \#75604}
\bigskip
I thank the referee for his/her constructive comments. I have tried to respond
all the referee's points in ``Responses to the referee's report", and made
the necessary modifications in the text.

======================================

   				RESPONSES TO THE REFEREE'S REPORT

======================================
(1) In Figure 6, one sees that an "MRI-type wave" is excited by noise at the upper boundary and propagates downwards. When the velocity profile is switched to the ideal Couette flow, the waves very slowly fade away. The author calls these waves "inertial oscillations". However, they clearly have the same properties as the earlier "MRI-waves", which in turn look very similar to the "MRI-type waves" observed in the various versions of PROMISE. What I am getting at is the following : Wei Liu emphasizes that the threshold for absolute instability is not reached in PROMISE II, and he is probably right; however, the properties of the waves observed in the experiment are probably identical to those that would develop beyond the threshold. I suggest that the author discusses this question somewhat. 

Yes, the speculation of the referee is right. In order to clarify this point more clearly, the Fig. 6 is replaced by a extended version (the time frame is extended from $2000\;\units}$ to $3000\;\unit{s}$), which shows the inertial oscillation fades away completely due to the viscous diffusion. The similarity between these "inertial-oscillation-induced wave" after the switch and the earlier noise-sustained "MRI-waves" in the simulation or "MRI-type waves" observed in the various versions of PROMISE stems from the physical nature of HMRI that HMRI is a weakly destabilized inertial oscillation [Liu et al, PRE 74, 056302 (2006)]. More importantly, this similarity supports our conclusion in another aspect: the frequency and wave number selection mechanism for a noise-sustained structure is determined by a linear mechanism, thus resembling the properties of the primary instability. In contrast in the globally unstable regime, a nonlinear eigenvalue problem selects the frequency [Proctor et al, Physica D 145, 191 (2000)]. 

(2) Also, since m=1 waves are observed in the experiments, while they are excluded from the analysis of Wei Liu, one would like to know if a lower threshold could be obtained for this symmetry.

Yes, definitely m=1 mode is an interesting question. As stated by the referee, since the simulation presented in this paper is axisymmetric, the possibility to study this important mode is excluded. The extension of the current work to 3D will be the subject of the future study. Ruediger et al have already done some excellent work on this issue and found that given PROMISE parameters the nonaxisymmetric HMRI modes are always harder to be excited than the symmetric mode [Ruediger and Schultz, Astron. Nachr. 329, 659 (2008), Ruediger et al, Astron. Nachr. 326, 409 (2005)].

(3) A final, maybe naive, question : Wei Liu proposes a rough extrapolation of the actual threshold for the HMRI with an ideal Couette profile. Can he run his axisymmetric code in this regime and check this prediction?

This is certainly not a naive question, but rather an excellent question. Actually I tried to do the same thing as suggested by the referee. However I met with the following problems: (1)~the current code can not afford large Reynolds number ($\sim\times10^5$), which is required for HMRI to enter the absolutely unstable regime; (2)~from the global linear calculation, the HMRI mode is stabilized if an artificially low Reynolds number like $\sim10^3$, which could be afforded by the current code, is employed. Given the above constraints, I gave up this trial. 

(4) Reference Update
I have added three references: one for the relevance of absolute v.s. convective instability to Riga dynamo [Gailitis et al,  Comtes Rendus Physique 9, 721 (2008)], one for the introduction and recent results of PROMISE II [Stefani et al, arXiv:0807.0299] and one for importance of the distinction between absolute and convective instability in the context of the HMRI [Priede and Gerbeth, arXiv:0810.0386]. 


 
\bye
